Overcoming Pedestrian Blockage in mm-Wave Bands using Ground Reflections

mm-Wave communication employs directional beams to overcome high path loss. High data rate communication is typically along line-of-sight (LoS). In outdoor environments, such communication is susceptible to temporary blockage by pedestrians interposed between the transmitter and receiver. It results in outages in which the user is lost, and has to be reacquired as a new user, severely disrupting interactive and high throughput applications. It has been presumed that the solution is to have a densely deployed set of base stations that will allow the mobile to perform a handover to a different non-blocked base station every time a current base station is blocked. This is however a very costly solution for outdoor environments. Through extensive experiments we show that it is possible to exploit a strong ground reflection with a received signal strength (RSS) about 4dB less than the LoS path in outdoor built environments with concrete or gravel surfaces, for beams that are narrow in azimuth but wide in zenith. While such reflected paths cannot support the high data rates of LoS paths, they can support control channel communication, and, importantly, sustain time synchronization between the mobile and the base station. This allows a mobile to quickly recover to the LoS path upon the cessation of the temporary blockage, which typically lasts a few hundred milliseconds. We present a simple in-band protocol that quickly discovers ground reflected radiation and uses it to recover the LoS link when the temporary blockage disappears.

==> Blockage.tex <==
How to overcome blockage
What is that mobile needs from the base station
How to estimate those parameters
How to inform base station angle and tilt
Why do we need to that
Is it still necessary to get ambient in

==> Section1.tex <==
\section{Main Ideas}
Blockage is a fundamental problem for the success of mm-wave networks.\\
How antenna beam looks like zenith vs azimuth. why people looked in azimuth steering, which basically helped them ignore the ground reflections.\\
What other works did, why what did is different.\\
How to formalize our observation into a mathematical expression.\\ 
Most of works look into the environment scatters and ignored the ground reflections, so explored\\
Measurement model, experiments-- different surfaces, indoor and outdoors.\
Either indoor or outdoor\\
Blockage detection\\
Protocol to look into the block-- estimate distance to base station from base station-- What is base station responsible for, how UE should overcome the problem\\
Suggestion for cost effective deployments.
Comparison with other works-- Unblock, BeamSpy, Facilitating robust 60 ghz
network deployment by sensing ambient reflectors \\
Plot azimuth observation for each surface -- 3 plots and base station tilts
No prior work to address blockage in outdoor scenarios other than increasing blockage density.

